Exploiting Null Space in Aerial Manipulation through Model-In-The-Loop Motion Planning

This paper presents a method for aerial manipulator end-effector trajectory tracking by encompassing dynamics of the Unmanned Aerial Vehicle (UAV) and null space of the manipulator attached to it in the motion planning procedure. The proposed method runs in phases. Trajectory planning starts by not accounting for roll and pitch angles of the underactuated UAV system. Next, we propose simulating the dynamics on such a trajectory and obtaining UAV attitude through the model. The full aerial manipulator state obtained in such a manner is further utilized to account for discrepancies in planned and simulated end-effector states. Finally, the end-effector pose is corrected through the null space of the manipulator to match the desired end-effector pose obtained in trajectory planning. Furthermore, we have applied the TOPP-RA approach on the UAV by invoking the differential flatness principle. Finally, we conducted experimental tests to verify effectiveness of the planning framework.

==> content/simulation.tex <==
\section{Simulation}
\todo[inline]{Gazebo, realistično, citirati eth i hector.}
\todo[inline]{Opisati da smo napravili identifikaciju modela iz simulacije(iako ga znamo u potpunosti morali smo isprobati bla bla), Matlab model za simulaciju dinamike}
